Global SLAM Using 5G ToA Integration: Performance Analysis with Unknown Base Stations and Loop Closure Alternatives

This paper presents a novel approach that integrates 5G Time of Arrival (ToA) measurements into ORB-SLAM3 to enable global localization and enhance mapping capabilities for indoor drone navigation. We extend ORB-SLAM3's optimization pipeline to jointly process ToA data from 5G base stations alongside visual and inertial measurements while estimating system biases. This integration transforms the inherently local SLAM estimates into globally referenced trajectories and effectively resolves scale ambiguity in monocular configurations. Our method is evaluated using both Aerolab indoor datasets with RGB-D cameras and the EuRoC MAV benchmark, complemented by simulated 5G ToA measurements at 28 GHz and 78 GHz frequencies using MATLAB and QuaDRiGa. Extensive experiments across multiple SLAM configurations demonstrate that ToA integration enables consistent global positioning across all modes while maintaining local accuracy. For monocular configurations, ToA integration successfully resolves scale ambiguity and improves consistency. We further investigate scenarios with unknown base station positions and demonstrate that ToA measurements can effectively serve as an alternative to loop closure for drift correction. We also analyze how different geometric arrangements of base stations impact SLAM performance. Comparative analysis with state-of-the-art methods, including UWB-VO, confirms our approach's robustness even with lower measurement frequencies and sequential base station operation. The results validate that 5G ToA integration provides substantial benefits for global SLAM applications, particularly in challenging indoor environments where accurate positioning is critical.

==> sections/exp_old.tex <==
\section{Experiment}
\label{sec:experiments}
This section presents a detailed evaluation of the proposed methodology. Our experiments are designed to assess the performance of the SLAM system under diverse configurations, focusing on integrating simulated 5G ToA measurements with traditional visual and inertial data. The results provide insights into the impact of ToA integration across multiple datasets, sensor configurations, and 5G frequency bands.







\subsection{Experimental Setup and Data Collection}
The experiments were conducted in a controlled indoor environment, the Aerolab, specifically designed to support drone flights and data collection under realistic conditions for SLAM evaluation. The core equipment included an Intel RealSense D435i camera, used for RGB-D (color and depth) and IMU data acquisition, and the OptiTrack motion capture system, which provided high-precision ground truth data through a 12-camera configuration. Integrating these components enabled a comprehensive setup for acquiring synchronized data essential for SLAM.

The Intel RealSense D435i camera, mounted on the drone, captured RGB-D data at 30 Hz and IMU data at 200 Hz, with automatic synchronization between the visual and inertial data streams. To further support SLAM evaluation, five unique datasets were collected by flying the drone through varied trajectories that mimic realistic navigation scenarios, capturing a wide range of motion. Additionally, simulated 5G ToA data was generated at a rate of 10 Hz to complement the visual and inertial data. OptiTrack ground truth data was collected at 120 Hz, ensuring high accuracy and alignment with the other sensor modalities.

The drone operated within a netted 5x5x5 meter flight area for safety, though the Aerolab itself is larger, providing additional space for equipment and experimental setups. Each dataset represents a different flight path and duration, as detailed below:
\begin{itemize}
    \item \textbf{Dataset 0}: 116 seconds
    \item \textbf{Dataset 1}: 110 seconds
    \item \textbf{Dataset 2}: 135 seconds
    \item \textbf{Dataset 3}: 124 seconds
    \item \textbf{Dataset 4}: 139 seconds
\end{itemize}

The trajectories for each dataset are visualized in Figure~\ref{fig:gt_traj}, where the top row displays the x-y trajectories and the bottom row illustrates the time vs. z plots. 

\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{gt0}
        \caption{Dataset0}
        \label{fig:gt0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{gt1}
        \caption{Dataset1}
        \label{fig:gt1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{gt2}
        \caption{Dataset2}
        \label{fig:gt2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{gt3}
        \caption{Dataset3}
        \label{fig:gt3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\linewidth]{gt4}
        \caption{Dataset4}
        \label{fig:gt4}
    \end{subfigure}
    \caption[Trajectories for the five AeroLab datasets]{Trajectories for the five Aerolab datasets. Each subfigure contains the x-y trajectory (top) and the time vs. z trajectory (bottom) for a specific dataset.}
    \label{fig:gt_traj}
\end{figure*}


The setup, including the drone equipped with the RealSense camera and the Aerolab environment, is illustrated in Figure~\ref{fig:three_images}. This figure provides visual context for the controlled flight space and the comprehensive equipment layout used for data collection.

The experiments were performed on a Ubuntu 20.04 laptop equipped with an Intel(R) Core(TM) i9-10885H CPU @ 2.40GHz with 16 cores and 32 GB of RAM. 

In addition to the Aerolab datasets, we extended our evaluation to include the EuRoC MAV benchmark dataset \cite{burri2016euroc}, which is widely used for SLAM performance assessment. For the Machine Hall sequences (MH01-MH05), we used a simple Gaussian simulation of ToA measurements to enable direct comparison with UWB-VO under identical conditions. However, for the Vicon Room sequences (V101-V203), we employed our comprehensive 5G ToA simulation methodology as detailed in \cite{kabiri2023pose, kabiri2024graph}, including realistic channel modeling with QuaDRiGa. The EuRoC MAV dataset provides stereo images, IMU measurements, and precise ground truth from a Vicon motion capture system across various indoor environments with different complexity levels, making it ideal for benchmarking our approach against existing methods.

To evaluate system robustness, we introduced significant noise to initial transformation estimates: 0.5m translation and $30^{\circ}$ rotation for MONO mode, and 1m translation with $90 ^{\circ}$  rotation for other modes. These substantial uncertainties effectively test the system's trajectory recovery capabilities,  simulating real-world scenarios where initial estimates may be imprecise.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{drone.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{drone2.png}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{aero_field.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{aero_full.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}



\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{drone2.png}
        \caption{Drone Setup}
        \label{fig:drone2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{aero_field.jpg}
        \caption{Flight area}
        \label{fig:aero_field}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{aero_full.jpg}
        \caption{Aerolab overview}
        \label{fig:aero_full}
    \end{subfigure}
    \caption[Drone setup, flight area, and Aerolab overview]{(a) Drone equipped with an Intel RealSense D435i camera for RGB-D and IMU data acquisition. (b) Experimental flight area within the netted environment for safe indoor drone testing. (c) Overall view of the Aerolab, illustrating both the drone testing area and additional laboratory equipment and space.}
    \label{fig:three_images}
\end{figure*}





\subsection{Calibration and Data Synchronization}
For the Aerolab datasets, the intrinsic and extrinsic calibration of the camera and IMU was conducted using the \texttt{Kalibr} toolbox and \texttt{allan\_variance\_ros}. The calibration procedure involved collecting data with checkerboard patterns and performing specific drone motions. This process resulted in intrinsic parameters such as focal length and distortion coefficients, as well as the transformation matrix between the camera and IMU, crucial for accurate sensor fusion.
Data synchronization is essential for optimal SLAM performance. Since the RealSense camera provides both RGB-D and IMU data, these streams are automatically synchronized. The OptiTrack system's ground truth data is also time-aligned with the collected data. The 5G ToA measurements are simulated based on the OptiTrack trajectories, ensuring that all datasets are synchronized.


\subsection{Augmenting Dataset with Simulated 5G ToA Measurements}

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.9\linewidth]{system_arch_slam.pdf}
    \caption[Dataset generation pipeline for 5G-enhanced SLAM]{Architecture of the dataset generation pipeline, showing the integration of simulated 5G ToA measurements with the Aerolab dataset. The pipeline consists of a 5G signal simulator using QuaDRiGa channel models, signal processing components (correlator and peak detection), and the final integration with IMU and image data from the Aerolab dataset. The combined data serves as input to the SLAM framework, with ToA measurements scaled by the speed of light to obtain distance measurements.}
    \label{fig:slam_architecture}
\end{figure*}
Acquiring real 5G ToA data in our lab setting is constrained by infrastructure and hardware limitations. To overcome this barrier, we employ a simulation-based approach to generate realistic ToA measurements. This strategy enables us to assess the advantages of integrating 5G positioning signals into the SLAM framework without the need for extensive physical network setups. By combining simulated ToA data with authentic drone flight data that includes RGB-D images, IMU readings, and precise ground truth trajectories, we construct an augmented dataset suitable for SLAM performance assessment. Figure~\ref{fig:slam_architecture} illustrates the overall structure of the simulation environment and how its components interact to generate this augmented dataset.







\subsection{5G ToA Simulation Methodology}
Following our previous work \cite{kabiri2024graph}, we employ the same rigorous methodology to simulate 5G ToA measurements for the current dataset under the line-of-sight condition. The simulation framework utilizes the MATLAB 5G Toolbox to generate 5G signals, including Positioning Reference Signals (PRS) and Physical Downlink Shared Channel (PDSCH) resources, with consistent transmission parameters (0 dBm transmit power and 10 dB SNR).

The wireless channel characteristics are simulated using QuaDRiGa (quasi-deterministic radio channel generator) \cite{jaeckel2017quadriga} with two distinct 5G FR2 (millimeter wave) network configurations: a 28 GHz configuration utilizing 200 MHz channel bandwidth with 120 kHz subcarrier spacing, and a 78 GHz configuration employing 400 MHz channel bandwidth with 240 kHz subcarrier spacing, both aligning with 3GPP specifications for FR2 deployments.

While the simulation framework remains unchanged, we adapt the base station placement to suit the current dataset's environment. We virtually position four BSs within the experimental space, with coordinates defined in the OptiTrack system's global frame as:
BS1: $(2.5, -2.5, 4.5)$, 
BS2: $(2.5, 2.5, 4.0)$, 
BS3: $(-2.5, 2.5, 5.0)$, 
BS4: $(-6.5, -2.5, 2.0)$. The receiver is also assumed to be mounted on top of the drone. 





The simulation maintains the established configuration parameters:

\begin{itemize}
\item Signal generation at 10 Hz (every 0.1 seconds)
\item Empirically validated correlation threshold of 0.2 for ToA estimation
\item Omnidirectional antenna configurations for both transmitters and receivers
\item Consistent 5G system parameters across scenarios (bandwidth, subcarrier spacing, resource blocks, comb size, and cyclic prefix type)
\end{itemize}

The trajectory data from the current dataset is processed by computing velocities from consecutive pose measurements to maintain compatibility with the QuaDRiGa channel simulator's requirements. This ensures that the simulated ToA measurements accurately reflect the dynamic characteristics of the platform's motion in the new environment while maintaining consistency with our validated simulation methodology. The final statistics of the simulated ToA are given in Table \ref{tab:toa_detailed_summary}. 



\begin{table}[ht]
    \centering
    \caption[ToA stats for 28 GHz and 78 GHz across datasets and base stations]{ToA Mean and Standard Deviation for 28 GHz and 78 GHz Frequencies Across Five Datasets and Four Base Stations}
    \label{tab:toa_detailed_summary}
    \begin{adjustbox}{width=1\linewidth}
    \scriptsize
    \begin{tabular}{
        l        % Dataset
        c        % Frequency (GHz)
        c        % Base Station
        S[table-format=2.2] % Std (cm)
        S[table-format=2.2] % Mean (cm)
    }
    \toprule
    \textbf{Dataset} & \textbf{Frequency (GHz)} & \textbf{Base Station} & \textbf{Std (cm)} & \textbf{Mean (cm)} \\
    \midrule
    \multirow{8}{*}{Dataset0} 
        & \multirow{4}{*}{28} 
            & \cellcolor{lightgray}1 & \cellcolor{lightgray}32.92 & \cellcolor{lightgray}4.20 \\
        &                       & 2 & 36.05 & -1.21 \\
        &                       & \cellcolor{lightgray}3 & \cellcolor{lightgray}31.99 & \cellcolor{lightgray}4.19 \\
        &                       & 4 & 41.32 & 8.28 \\
        \cmidrule(lr){2-5}
        & \multirow{4}{*}{78} 
            & \cellcolor{lightgray}1 & \cellcolor{lightgray}19.58 & \cellcolor{lightgray}-2.71 \\
        &                       & 2 & 19.44 & 1.34 \\
        &                       & \cellcolor{lightgray}3 & \cellcolor{lightgray}19.10 & \cellcolor{lightgray}0.31 \\
        &                       & 4 & 14.25 & -1.72 \\
    \midrule
    \multirow{8}{*}{Dataset1} 
        & \multirow{4}{*}{28} 
            & \cellcolor{lightgray}1 & \cellcolor{lightgray}36.31 & \cellcolor{lightgray}-6.88 \\
        &                       & 2 & 29.60 & -3.56 \\
        &                       & \cellcolor{lightgray}3 & \cellcolor{lightgray}36.60 & \cellcolor{lightgray}1.88 \\
        &                       & 4 & 32.22 & -2.68 \\
        \cmidrule(lr){2-5}
        & \multirow{4}{*}{78} 
            & \cellcolor{lightgray}1 & \cellcolor{lightgray}15.95 & \cellcolor{lightgray}-2.83 \\
        &                       & 2 & 17.01 & -2.29 \\
        &                       & \cellcolor{lightgray}3 & \cellcolor{lightgray}16.08 & \cellcolor{lightgray}0.56 \\
        &                       & 4 & 15.64 & -0.86 \\
    \midrule
    \multirow{8}{*}{Dataset2} 
        & \multirow{4}{*}{28} 
            & \cellcolor{lightgray}1 & \cellcolor{lightgray}38.44 & \cellcolor{lightgray}-8.24 \\
        &                       & 2 & 31.94 & -4.93 \\
        &                       & \cellcolor{lightgray}3 & \cellcolor{lightgray}33.25 & \cellcolor{lightgray}7.97 \\
        &                       & 4 & 30.49 & -0.50 \\
        \cmidrule(lr){2-5}
        & \multirow{4}{*}{78} 
            & \cellcolor{lightgray}1 & \cellcolor{lightgray}15.83 & \cellcolor{lightgray}0.87 \\
        &                       & 2 & 18.92 & -4.97 \\
        &                       & \cellcolor{lightgray}3 & \cellcolor{lightgray}16.38 & \cellcolor{lightgray}-0.80 \\
        &                       & 4 & 16.63 & -0.59 \\
    \midrule
    \multirow{8}{*}{Dataset3} 
        & \multirow{4}{*}{28} 
            & \cellcolor{lightgray}1 & \cellcolor{lightgray}40.14 & \cellcolor{lightgray}-14.56 \\
        &                       & 2 & 32.19 & -6.68 \\
        &                       & \cellcolor{lightgray}3 & \cellcolor{lightgray}31.17 & \cellcolor{lightgray}4.49 \\
        &                       & 4 & 27.64 & -4.97 \\
        \cmidrule(lr){2-5}
        & \multirow{4}{*}{78} 
            & \cellcolor{lightgray}1 & \cellcolor{lightgray}15.03 & \cellcolor{lightgray}0.87 \\
        &                       & 2 & 17.61 & -8.71 \\
        &                       & \cellcolor{lightgray}3 & \cellcolor{lightgray}14.69 & \cellcolor{lightgray}-1.49 \\
        &                       & 4 & 15.94 & -1.06 \\
    \midrule
    \multirow{8}{*}{Dataset4} 
        & \multirow{4}{*}{28} 
            & \cellcolor{lightgray}1 & \cellcolor{lightgray}38.23 & \cellcolor{lightgray}-19.41 \\
        &                       & 2 & 29.54 & -2.18 \\
        &                       & \cellcolor{lightgray}3 & \cellcolor{lightgray}31.23 & \cellcolor{lightgray}-3.09 \\
        &                       & 4 & 40.62 & -8.31 \\
        \cmidrule(lr){2-5}
        & \multirow{4}{*}{78} 
            & \cellcolor{lightgray}1 & \cellcolor{lightgray}14.40 & \cellcolor{lightgray}3.12 \\
        &                       & 2 & 16.80 & -4.67 \\
        &                       & \cellcolor{lightgray}3 & \cellcolor{lightgray}15.56 & \cellcolor{lightgray}0.57 \\
        &                       & 4 & 18.76 & -1.08 \\
    \bottomrule
    \end{tabular}%
    \end{adjustbox}
\end{table}

That table reveals differences between the two frequency bands across all datasets. The 78 GHz configuration demonstrates superior precision with standard deviations ranging from 14.25-19.58 cm, compared to the 28 GHz measurements which show larger variations of 27.64-41.32 cm. Mean errors at 78 GHz typically remain within ±5 cm, while 28 GHz measurements exhibit larger systematic biases up to 19.41 cm. The 78 GHz configuration's superior performance, evidenced by approximately 50\% lower standard deviation and smaller systematic biases across all datasets, suggests it is the preferred choice for precise ToA measurements in indoor drone navigation scenarios. This performance advantage can be attributed to the larger bandwidth (400 MHz vs 200 MHz) and higher subcarrier spacing (240 kHz vs 120 kHz) available at 78 GHz.


\subsection{Evaluation Metrics}
We evaluated the system using the Absolute Trajectory Error (ATE) metric, comparing the estimated trajectories against the OptiTrack system's ground truth. Two distinct evaluation approaches were employed:

\begin{itemize}
    \item Local Evaluation: Before computing the ATE, we estimate and apply an optimal transformation (rotation, translation, and scale) between the SLAM-estimated trajectory and the ground truth. This alignment process factors out global positioning errors and evaluates the system's ability to maintain consistent local trajectory shape and motion patterns. For example, if the drone flies in a square pattern, this evaluation would measure how well the SLAM system captures the square's shape, regardless of its absolute position or orientation in space.
    \item Global Evaluation: No transformation or scale optimization was applied, enabling direct comparison between estimated and ground truth trajectories in their original coordinate frames. This approach provides a stringent assessment of the system's ability to maintain accurate absolute positioning and orientation across the entire flight path.
\end{itemize}




Both evaluations were compared against the baseline ORB-SLAM3 system without ToA data integration, demonstrating how 5G measurements enhance global positioning capabilities while preserving local consistency.























==> sections/results_old.tex <==

\section{Results}
\label{sec:resuls}

In this section, we present the experimental results that evaluate the performance of different SLAM modes integrated with 5G ToA data at two frequencies: 28 GHz and 78 GHz. Table \ref{tab:combined} presents comprehensive performance metrics for four SLAM configurations: RGB-D, RGB-D Inertial, Monocular (MONO), and Monocular Inertial. The results are evaluated across five distinct datasets (Dataset0 through Dataset4) collected in the Aerolab environment. For each configuration and dataset, we report three key metrics: local error (in meters), global error (in meters), and local improvement percentage compared to the baseline. To ensure statistical reliability, each experiment was conducted five times, and the values presented in the table represent the average ATE across these runs. The table includes both baseline measurements (without ToA integration) and results with ToA integration at both frequency bands, along with mode averages for each SLAM configuration. %For enhanced clarity and visual representation, Fig.\ref{fig:combined_barcharts} presents four bar charts illustrating the performance comparisons for the RGB-D, RGB-D Inertial, Monocular (MONO), and Monocular Inertial SLAM modes. These charts showcase the ATEs for both the baseline and the proposed ToA-integrated systems at 28~GHz and 78~GHz frequencies, with results evaluated under both local and global criteria across all datasets. The baseline global ATE values are omitted from the bar charts as they are significantly larger across all datasets, which would disproportionately scale the chart and reduce the visibility of the other results.




% \begin{table}[!h]
%     \centering
%     \caption{Average Errors for Different SLAM Modes. \\
%     \textit{Note: For the monocular mode with TOA integration, results for datasets 2 and 4 are calculated up to 75 seconds and 65 seconds respectively, as the system lost tracking beyond these durations.}}
%     \label{tab:combined}
%     \resizebox{0.95\linewidth}{!}{%
%         \begin{tabular}{l c l cc}
%             \toprule
%             \textbf{SLAM Mode} & \textbf{Dataset} & \textbf{Configuration} & \textbf{Local (m)} & \textbf{Global (m)} \\
%             \midrule
%             % RGB-D SLAM Mode
%             \multirow{15}{*}{RGB-D} 
%             & \multirow{3}{*}{\centering Dataset0} & Baseline & 0.064 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.066 & \cellcolor{lightgray}0.237 \\
%             & & 78 GHz ToA & 0.055 & 0.101 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset1} & Baseline & 0.116 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.117 & \cellcolor{lightgray}0.165 \\
%             & & 78 GHz ToA & 0.117 & 0.133 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset2} & Baseline & 0.155 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.160 & \cellcolor{lightgray}0.197 \\
%             & & 78 GHz ToA & 0.148 & 0.158 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset3} & Baseline & 0.095 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.102 & \cellcolor{lightgray}0.149 \\
%             & & 78 GHz ToA & 0.094 & 0.104 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset4} & Baseline & 0.146 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.162 & \cellcolor{lightgray}0.242 \\
%             & & 78 GHz ToA & 0.164 & 0.171 \\
%             \midrule
%             % RGB-D Inertial SLAM Mode
%             \multirow{15}{*}{RGB-D Inertial}
%             & \multirow{3}{*}{\centering Dataset0} & Baseline & 0.089 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.092 & \cellcolor{lightgray}0.471 \\
%             & & 78 GHz ToA & 0.075 & 0.276 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset1} & Baseline & 0.119 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.118 & \cellcolor{lightgray}0.206 \\
%             & & 78 GHz ToA & 0.118 & 0.315 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset2} & Baseline & 0.216 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.231 & \cellcolor{lightgray}0.267 \\
%             & & 78 GHz ToA & 0.366 & 0.426 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset3} & Baseline & 0.065 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.064 & \cellcolor{lightgray}0.134 \\
%             & & 78 GHz ToA & 0.062 & 0.125 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset4} & Baseline & 0.108 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.105 & \cellcolor{lightgray}0.321 \\
%             & & 78 GHz ToA & 0.105 & 0.168 \\
%             \midrule
%             % MONO SLAM Mode
%             \multirow{15}{*}{MONO}
%             & \multirow{3}{*}{\centering Dataset0} & Baseline & -- & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}-- & \cellcolor{lightgray}-- \\
%             & & 78 GHz ToA & -- & -- \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset1} & Baseline & 1.370 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.059 & \cellcolor{lightgray}0.380 \\
%             & & 78 GHz ToA & 0.058 & 0.121 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset2} & Baseline & 1.284 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.089 & \cellcolor{lightgray}0.186 \\
%             & & 78 GHz ToA & 0.075 & 0.152 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset3} & Baseline & 1.363 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.058 & \cellcolor{lightgray}0.162 \\
%             & & 78 GHz ToA & 0.058 & 0.127 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset4} & Baseline & 1.041 & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.179 & \cellcolor{lightgray}0.320 \\
%             & & 78 GHz ToA & 0.061 & 0.131 \\
%             \midrule
%             % MONO Inertial SLAM Mode
%             \multirow{15}{*}{MONO Inertial}
%             & \multirow{3}{*}{\centering Dataset0} & Baseline & -- & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.096 & \cellcolor{lightgray}0.434 \\
%             & & 78 GHz ToA & 0.076 & 0.306 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset1} & Baseline & -- & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.112 & \cellcolor{lightgray}0.190 \\
%             & & 78 GHz ToA & 0.121 & 0.370 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset2} & Baseline & -- & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.217 & \cellcolor{lightgray}0.336 \\
%             & & 78 GHz ToA & 0.197 & 0.649 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset3} & Baseline & -- & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.063 & \cellcolor{lightgray}0.128 \\
%             & & 78 GHz ToA & 0.063 & 0.123 \\
%             \cmidrule(lr){2-5}
%             & \multirow{3}{*}{\centering Dataset4} & Baseline & -- & -- \\
%             & & \cellcolor{lightgray}28 GHz ToA & \cellcolor{lightgray}0.102 & \cellcolor{lightgray}0.314 \\
%             & & 78 GHz ToA & 0.102 & 0.150 \\
%             \bottomrule
%         \end{tabular}
%     }
% \end{table}


% \begin{figure*}[!htb] % Use figure* to span both columns in two-column mode
%     \centering
%     % First Row: RGB-D and RGB-D-Inertial
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{barchart_rgbd.pdf}
%         \caption{RGB-D}
%         \label{fig:barchart_rgbd}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{barchart_RgbdInertial.pdf}
%         \caption{RGB-D-Inertial}
%         \label{fig:barchart_RgbdInertial}
%     \end{subfigure}
    
%     \vspace{0.5cm} % Adds vertical space between the two rows
    
%     % Second Row: Mono and Mono-Inertial
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{barchart_mono.pdf}
%         \caption{Mono}
%         \label{fig:barchart_mono}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{barchart_monoInertial.pdf}
%         \caption{Mono-Inertial}
%         \label{fig:barchart_monoInertial}
%     \end{subfigure}
    
%     \caption[Bar chart of ATEs for SLAM modes]{Bar charts comparing Absolute Trajectory Errors (ATEs) for SLAM modes (a) RGB-D, (b) RGB-D-Inertial, (c) Mono, and (d) Mono-Inertial with and without ToA integration at 28 GHz and 78 GHz. Results are evaluated using local and global criteria across five datasets.}
%     \label{fig:combined_barcharts}
% \end{figure*}


\begin{table}[!h]
    \centering
    \caption[Comparison of SLAM Performance with ToA Integration]{Average Errors and Improvements for Different SLAM Modes. \textit{\footnotesize Note: For the monocular mode with TOA integration, results for Datasets 2 and 4  are calculated up to 75\,s and 65\,s respectively, as the system lost tracking beyond these durations.}}
    \label{tab:combined}
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{l c l c c c}
        \toprule
        \textbf{SLAM Mode} & \textbf{Dataset} & \textbf{Configuration} 
          & \textbf{Local (m)} & \textbf{Global (m)} & \textbf{Local Imp.} \\
        \midrule
        
        % --------------------------- RGB-D SLAM Mode ---------------------------
        \multirow{18}{*}{RGB-D} 
        & \multirow{3}{*}{Dataset0} 
            & Baseline 
                & 0.064 & N/A$^\ddagger$    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.066 
                & \cellcolor{lightgray}0.237 
                & \cellcolor{lightgray}\coloredpercent{-3.1} \\
        &   & 78 GHz ToA
                & 0.055 & 0.101 & \coloredpercent{14.1} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset1} 
            & Baseline 
                & 0.116 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.117 
                & \cellcolor{lightgray}0.165 
                & \cellcolor{lightgray}\coloredpercent{-0.9} \\
        &   & 78 GHz ToA
                & 0.117 & 0.133 & \coloredpercent{-0.9} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset2} 
            & Baseline 
                & 0.155 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.160 
                & \cellcolor{lightgray}0.197 
                & \cellcolor{lightgray}\coloredpercent{-3.2} \\
        &   & 78 GHz ToA
                & 0.148 & 0.158 & \coloredpercent{4.5} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset3} 
            & Baseline 
                & 0.095 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.102
                & \cellcolor{lightgray}0.149
                & \cellcolor{lightgray}\coloredpercent{-7.4} \\
        &   & 78 GHz ToA
                & 0.094 & 0.104 & \coloredpercent{1.1} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset4} 
            & Baseline
                & 0.146 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.162
                & \cellcolor{lightgray}0.242
                & \cellcolor{lightgray}\coloredpercent{-11.0} \\
        &   & 78 GHz ToA
                & 0.164 & 0.171 & \coloredpercent{-12.3} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{\textbf{Mode Average}} 
            & Baseline
                & \textbf{0.115} & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}\textbf{0.121}
                & \cellcolor{lightgray}\textbf{0.198}
                & \cellcolor{lightgray}\textbf{\coloredpercent{-5.2}} \\
        &   & 78 GHz ToA
                & \textbf{0.116} & \textbf{0.133} & \textbf{\coloredpercent{1.3}} \\
        
        \midrule
        % --------------------- RGB-D Inertial SLAM Mode -----------------------
        \multirow{18}{*}{RGB-D Inertial}
        & \multirow{3}{*}{Dataset0} 
            & Baseline
                & 0.089 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.092
                & \cellcolor{lightgray}0.471
                & \cellcolor{lightgray}\coloredpercent{-3.4} \\
        &   & 78 GHz ToA
                & 0.075 & 0.276 & \coloredpercent{15.7} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset1} 
            & Baseline
                & 0.119 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.118
                & \cellcolor{lightgray}0.206
                & \cellcolor{lightgray}\coloredpercent{0.8} \\
        &   & 78 GHz ToA
                & 0.118 & 0.315 & \coloredpercent{0.8} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset2} 
            & Baseline
                & 0.216 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.231$^\dagger$
                & \cellcolor{lightgray}0.267
                & \cellcolor{lightgray}\coloredpercent{-6.9}  $^\dagger$ \\
        &   & 78 GHz ToA
                & 0.366$^\dagger$ & 0.426 & \coloredpercent{-69.4} $^\dagger$  \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset3} 
            & Baseline
                & 0.065 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.064
                & \cellcolor{lightgray}0.134
                & \cellcolor{lightgray}\coloredpercent{1.5} \\
        &   & 78 GHz ToA
                & 0.062 & 0.125 & \coloredpercent{4.6} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset4} 
            & Baseline
                & 0.108 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.105
                & \cellcolor{lightgray}0.321
                & \cellcolor{lightgray}\coloredpercent{2.8} \\
        &   & 78 GHz ToA
                & 0.105 & 0.168 & \coloredpercent{2.8} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{\textbf{Mode Average}} 
            & Baseline
                & \textbf{0.095} & N/A & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}\textbf{0.094}
                & \cellcolor{lightgray}\textbf{0.280}
                & \cellcolor{lightgray}\textbf{\coloredpercent{0.42}} \\
        &   & 78 GHz ToA
                & \textbf{0.090} & \textbf{0.262} & \textbf{\coloredpercent{5.97}} \\
        
        \midrule
        % --------------------------- MONO SLAM Mode ---------------------------
        \multirow{18}{*}{MONO}
        & \multirow{3}{*}{Dataset0} 
            & Baseline 
                & Failed    & N/A & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}Failed 
                & \cellcolor{lightgray}Failed
                & \cellcolor{lightgray}-- \\
        &   & 78 GHz ToA
                & Failed    & Failed & -- \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset1} 
            & Baseline
                & 1.370 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.059
                & \cellcolor{lightgray}0.380
                & \cellcolor{lightgray}\coloredpercent{95.7} \\
        &   & 78 GHz ToA
                & 0.058 & 0.121 & \coloredpercent{95.8} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset2} 
            & Baseline
                & 1.284 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.089
                & \cellcolor{lightgray}0.186
                & \cellcolor{lightgray}\coloredpercent{93.1} \\
        &   & 78 GHz ToA
                & 0.075 & 0.152 & \coloredpercent{94.2} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset3} 
            & Baseline
                & 1.363 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.058
                & \cellcolor{lightgray}0.162
                & \cellcolor{lightgray}\coloredpercent{95.7} \\
        &   & 78 GHz ToA
                & 0.058 & 0.127 & \coloredpercent{95.7} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset4} 
            & Baseline
                & 1.041 & N/A    & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.179
                & \cellcolor{lightgray}0.320
                & \cellcolor{lightgray}\coloredpercent{82.8} \\
        &   & 78 GHz ToA
                & 0.061 & 0.131 & \coloredpercent{94.1} \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{\textbf{Mode Average}} 
            & Baseline
                & \textbf{1.265} & N/A & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}\textbf{0.096}
                & \cellcolor{lightgray}\textbf{0.262}
                & \cellcolor{lightgray}\textbf{\coloredpercent{92.4}} \\
        &   & 78 GHz ToA
                & \textbf{0.063} & \textbf{0.133} & \textbf{\coloredpercent{95.0}} \\
        
        \midrule
        % -------------------- MONO Inertial SLAM Mode -------------------------
        \multirow{18}{*}{MONO Inertial}
        & \multirow{3}{*}{Dataset0} 
            & Baseline 
                & Failed & N/A & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.096
                & \cellcolor{lightgray}0.434
                & \cellcolor{lightgray}  \nagreenn \\
        &   & 78 GHz ToA
                & 0.076 & 0.306 &  \nagreen \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset1} 
            & Baseline 
                & Failed & N/A & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.112
                & \cellcolor{lightgray}0.190
                & \cellcolor{lightgray}  \nagreen \\
        &   & 78 GHz ToA
                & 0.121 & 0.370 &  \nagreen \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset2} 
            & Baseline 
                & Failed & N/A & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.217
                & \cellcolor{lightgray}0.336
                & \cellcolor{lightgray} \nagreen \\
        &   & 78 GHz ToA
                & 0.197 & 0.649 &  \nagreen \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset3} 
            & Baseline 
                & Failed & N/A & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.063
                & \cellcolor{lightgray}0.128
                & \cellcolor{lightgray} \nagreen \\
        &   & 78 GHz ToA
                & 0.063 & 0.123 &  \nagreen \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{Dataset4} 
            & Baseline 
                & Failed & N/A & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}0.102
                & \cellcolor{lightgray}0.314
                & \cellcolor{lightgray} \nagreen \\
        &   & 78 GHz ToA
                & 0.102 & 0.150 &  \nagreen \\
        \cmidrule(lr){2-6}
        
        & \multirow{3}{*}{\textbf{Mode Average}} 
            & Baseline
                & \textbf{Failed} & N/A & -- \\
        &   & \cellcolor{lightgray}28 GHz ToA
                & \cellcolor{lightgray}\textbf{0.118}
                & \cellcolor{lightgray}\textbf{0.280}
                & \cellcolor{lightgray}\textbf{ \nagreen} \\
        &   & 78 GHz ToA
                & \textbf{0.112} & \textbf{0.320} & \textbf{ \nagreen} \\
        
        \bottomrule
    \end{tabular}
    }
        \\[0.5em] 
\begin{minipage}{\linewidth}
        {\fontsize{5}{8} \selectfont
            $\dagger$ Dataset2's RGB-D Inertial with ToA results were excluded from average calculations due to anomalous degradation. \\[-0.5em]
            $*$ The symbol INF indicates cases where ToA enabled successful tracking when the baseline failed.\\[-0.5em]
            $\ddagger$ N/A denotes baseline systems without global positioning capability.}
    \end{minipage}
\end{table}



\subsection{Evaluation Methodology: Local vs. Global Alignment}

Before delving into the analysis, it is crucial to understand the difference between local and global evaluations and the implications of including baseline global results.

In the \textbf{local evaluation}, the transformation (rotation and translation) between the estimated trajectory and the ground truth is assumed to be unknown and is calculated offline after the SLAM process. This alignment is typically performed using methods like Horn's absolute orientation algorithm, which finds the best-fit transformation that minimizes the trajectory error. Essentially, the local evaluation focuses on the consistency of the trajectory shape, disregarding the absolute positioning and orientation in the global frame.

In contrast, the \textbf{global evaluation} does not perform any post-processing alignment. The SLAM algorithm must estimate both the trajectory and the transformation directly, operating entirely in the global coordinate frame. This approach is more challenging because it requires the SLAM system to maintain accurate global positioning and orientation throughout the operation without relying on offline corrections. This capability is demonstrated in the 3D plot shown in Fig.~\ref{fig:3d_global}, which showcases one experiment (Dataset 0). The RGB-D trajectory enhanced with 78 GHz ToA measurements in the global frame closely matches the ground truth, demonstrating how ToA integration enables consistent global positioning.


% In contrast, the \textbf{global evaluation} does not perform any post-processing alignment. The SLAM algorithm must estimate both the trajectory and the transformation directly, operating entirely in the global coordinate frame. This approach is more challenging because it requires the SLAM system to maintain accurate global positioning and orientation throughout the operation without relying on offline corrections. This challenge is highlighted in the 3D plots shown in Fig.\ref{fig:3d_comparison}, which showcase one experiment (Dataset 0).  Fig.\ref{fig:3dlocal} shows the baseline RGB-D trajectory in its local frame, highlighting the misalignment with real-world coordinates. In contrast, Fig.\ref{fig:3dglobal} presents the RGB-D trajectory enhanced with 78 GHz ToA measurements in the global frame, which closely matches the ground truth, demonstrating how ToA integration improves global consistency.

% Including the \textbf{baseline global results} in our analysis provides insight into the ability of the baseline ORB-SLAM3 algorithm to estimate the global transformation without external aids like ToA data. However, it is important to note that the baseline algorithm is not designed to estimate global transformations during runtime in the absence of such data. Consequently, the baseline global errors are significantly higher than the local errors, as shown in Table~\ref{tab:combined}.

% Comparing the baseline global results directly with the local results can be misleading or considered unfair because the baseline algorithm lacks the necessary information to perform global localization without external references. Therefore, when interpreting the results, one should consider the baseline global errors as a demonstration of the limitations of traditional SLAM algorithms in estimating absolute positions without additional data, rather than a direct performance comparison.



% \begin{figure}[!htbp]
%     \centering
%     \begin{subfigure}{0.4\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{rgbd.png}
%         \caption{Local estimate without alignment}
%         \label{fig:3dlocal}
%     \end{subfigure}
%     \hfill % Adds space between the subfigures
%     \begin{subfigure}{0.4\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{rgbd_toa.png}
%         \caption{Global estimate with ToA at 78 GHz}
%         \label{fig:3dglobal}
%     \end{subfigure}
%     \caption[Local vs. global SLAM estimates with ToA integration]{Comparison of RGB-D trajectory and map point estimates in local and global frames for Dataset0. 
%     The SLAM results show keyframe pose estimates (blue lines), mapped features (black dots), and the ground truth trajectory (red line). Coordinate axes are color-coded: red for X, green for Y, and blue for Z. The local estimate (a) operates within the SLAM system’s frame, without real-world alignment. The global estimate (b), enhanced with 80 GHz ToA data, aligns closely with the ground truth in the global frame, demonstrating improved accuracy.}
%     \label{fig:3d_comparison}
% \end{figure}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{rgbd_toa.png}
    \caption[Global SLAM estimate with ToA integration]{RGB-D trajectory and map point estimates in the global frame for Dataset0 with 78 GHz ToA integration. 
    The SLAM results show keyframe pose estimates (blue lines), mapped features (black dots), and the ground truth trajectory (red line). Coordinate axes are color-coded: red for X, green for Y, and blue for Z. The trajectory estimate, enhanced with 78 GHz ToA data, aligns closely with the ground truth in the global frame, demonstrating the system's ability to maintain accurate global positioning without post-processing alignment.}
    \label{fig:3d_global}
\end{figure}


\subsection{Analysis of SLAM Modes with ToA Integration}

\subsubsection{RGB-D and RGB-D Inertial Modes}

For RGB-D SLAM mode, the baseline achieves exceptional local accuracy. Integrating 78 GHz ToA measurements shows slight improvements in most cases, while 28 GHz ToA integration results in minor degradation. This performance difference stems from two factors:

\begin{itemize}
    \item \textbf{Baseline Superiority and 6-DoF Interpretation:} the baseline's local accuracy already exceeds ToA measurement precision as shown in Table~\ref{tab:toa_detailed_summary}.  Additionally, ToA data offers only distance information, and translating these measurements into full 6-DoF pose estimations can inherently limit accuracy.

    \item \textbf{Post-Hoc Alignment and Fusion Complexity:} Post-hoc alignment compensates for global positioning errors, minimizing the impact of ToA integration on local accuracy. Furthermore, fusing additional sensor data introduces complexities and potential calibration challenges, which can lead to minor inconsistencies in the local ATEs.

\end{itemize}


For global evaluation, ToA integration effectively enables global localization, with 78 GHz measurements achieving global ATEs of approximately 0.1m on Dataset0, showcasing excellent performance and demonstrating robust global localization capabilities.

In the RGB-D Inertial mode, a similar pattern emerges. ToA integration offers modest improvements in local accuracy while enabling efficient global SLAM, addressing the limitations of the baseline, which lacks external references for global positioning.


\subsubsection{Monocular (MONO) Modes}

For {\textbf{MONO SLAM}} mode, the baseline encounters fundamental challenges due to scale ambiguity and the absence of depth information, leading to high ATEs and complete failure on Dataset 0. Even with post-hoc alignment, local errors remain above 1m, highlighting the limitations of the baseline approach.

The integration of ToA offers critical scale and positioning information, resulting in substantial performance improvements. At 78 GHz, global ATEs achieve an accuracy of 0.121m on Dataset 1. Local performance also benefits significantly, primarily due to enhanced scale and transformation estimation during SLAM operations, enabling more robust and reliable localization.



\subsubsection{Monocular Inertial Modes}


For \textbf{MONO Inertial} mode, the baseline fails across all datasets due to the compounding effects of inertial sensor noise. ToA integration significantly enhances both accuracy and robustness by enabling reliable scale and global transformation estimation while stabilizing the fusion of inertial data. At 78 GHz, global ATE achieves 0.123m on Dataset 3, demonstrating the potential of ToA integration in improving performance.

However, challenges persist in certain scenarios. For example, Dataset 2 exhibits a high global ATE of 0.649m even with 78 GHz ToA data. This highlights that while ToA integration addresses many limitations, effectively managing multiple sensor modalities under diverse conditions remains a complex task requiring further optimization.

\subsection{Impact of 5G Network Frequency on ToA Performance}

While the \textbf{78 GHz} 5G network configuration generally enables better ToA-based localization performance compared to \textbf{28 GHz} in the global evaluation, thanks to its greater bandwidth and subcarrier spacing, this pattern isn't universal across datasets. Performance variations between the two configurations may arise from measurement noise and ToA estimation accuracy under different conditions.

In the local evaluation, differences between the two 5G network configurations are less pronounced due to the effects of post-hoc alignment. However, the improved precision of the 78 GHz configuration often results in better trajectory consistency in most scenarios.




\subsection{Real-Time Performance}
Our approach achieves real-time operation on ROS bag files at normal playback speed, running on a laptop with Intel i9-10885H CPU (2.40GHz, 16 cores) and 32GB RAM under Ubuntu 20.04. This computational efficiency makes the system practical for real-time drone navigation applications.




\subsection{Summary and Key Findings}

The integration of ToA measurements with various SLAM configurations reveals distinct effects on both global and local performance. Most importantly, ToA integration addresses a fundamental limitation of traditional SLAM systems by enabling global localization capabilities, which are otherwise unattainable without external references. 

In minimal sensor configurations, such as Monocular SLAM, ToA integration proves transformative. Baseline Monocular SLAM suffers from scale ambiguity and significant trajectory errors, leading to local errors exceeding 1 meter even after scale correction. With ToA integration, the system achieves substantial improvements, with average local accuracies across datasets reaching 9.6 cm with 28 GHz and 6.3 cm with 78 GHz, notably outperforming the RGB-D SLAM baseline of 11.5 cm. Similarly, Monocular Inertial SLAM, which fails entirely in its baseline configuration, becomes fully operational with ToA integration, achieving average local accuracies around 11 cm across both frequency bands.

Conversely, for sensor-rich configurations like RGB-D SLAM, where the baseline already achieves high precision (around 11.5cm local error), ToA integration offers limited benefits for local accuracy. The 78 GHz configuration shows a modest 1.3\% improvement, while 28 GHz integration slightly degrades performance by 5.2\%. This pattern suggests that ToA measurements, while valuable for global positioning, may introduce additional noise that impacts local accuracy when combined with already precise depth measurements.
An interesting observation is the superior performance of 78 GHz ToA integration compared to 28 GHz across most configurations, particularly in global accuracy. This aligns with the theoretical advantages of higher frequency bands offering greater bandwidth and improved measurement precision. However, the performance gap between frequencies becomes less pronounced in local accuracy evaluation due to the effects of post-hoc alignment.

These findings highlight that ToA integration's impact is most beneficial in scenarios with minimal sensor configurations or when global positioning capabilities are required, while its utility for local accuracy may be limited in setups with high-precision depth sensing.











==> sections/table_slam_modes.tex <==
% \begin{table}[htbp]
%     \centering
%     \caption{Average Errors for Different SLAM Modes}
%     \label{tab:combined}

%     % First Row of Subtables
%     \begin{subtable}{0.45\textwidth}
%         \centering
%         \caption{RGB-D}
%         \resizebox{\linewidth}{!}{%
%         \begin{tabular}{c l cc}
%             \toprule
%             \textbf{Dataset} & \textbf{Configuration} & \textbf{Local (m)} & \textbf{Global (m)} \\
%             \midrule
%             \multirow{3}{*}{\centering Dataset0} & Baseline & 0.064 & 2.857 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.066 & \cellcolor{lightgray}0.237 \\
%             & 78 GHz \toa & 0.055 & 0.101 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset1} & Baseline & 0.116 & 2.739 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.117 & \cellcolor{lightgray}0.165 \\
%             & 78 GHz \toa & 0.117 & 0.133 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset2} & Baseline & 0.155 & 2.930 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.160 & \cellcolor{lightgray}0.197 \\
%             & 78 GHz \toa & 0.148 & 0.158 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset3} & Baseline & 0.095 & 2.594 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.102 & \cellcolor{lightgray}0.149 \\
%             & 78 GHz \toa & 0.094 & 0.104 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset4} & Baseline & 0.146 & 3.333 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.162 & \cellcolor{lightgray}0.242 \\
%             & 78 GHz \toa & 0.164 & 0.171 \\
%             \bottomrule
%         \end{tabular}
%         }
%     \end{subtable}
%     \hfill
%     \begin{subtable}{0.45\textwidth}
%         \centering
%         \caption{RGB-D Inertial}
%         \resizebox{\linewidth}{!}{%
%         \begin{tabular}{c l cc}
%             \toprule
%             \textbf{Dataset} & \textbf{Configuration} & \textbf{Local (m)} & \textbf{Global (m)} \\
%             \midrule
%             \multirow{3}{*}{\centering Dataset0} & Baseline & 0.089 & 1.467 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.092 & \cellcolor{lightgray}0.471 \\
%             & 78 GHz \toa & 0.075 & 0.276 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset1} & Baseline & 0.119 & 2.240 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.118 & \cellcolor{lightgray}0.206 \\
%             & 78 GHz \toa & 0.118 & 0.315 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset2} & Baseline & 0.216 & 1.964 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.231 & \cellcolor{lightgray}0.267 \\
%             & 78 GHz \toa & 0.366 & 0.426 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset3} & Baseline & 0.065 & 2.067 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.064 & \cellcolor{lightgray}0.134 \\
%             & 78 GHz \toa & 0.062 & 0.125 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset4} & Baseline & 0.108 & 1.947 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.105 & \cellcolor{lightgray}0.321 \\
%             & 78 GHz \toa & 0.105 & 0.168 \\
%             \bottomrule
%         \end{tabular}
%         }
%     \end{subtable}

%     \vspace{0.5cm}

%     % Second Row of Subtables
%     \begin{subtable}{0.45\textwidth}
%         \centering
%         \caption{MONO}
%         \resizebox{\linewidth}{!}{%
%         \begin{tabular}{c l cc}
%             \toprule
%             \textbf{Dataset} & \textbf{Configuration} & \textbf{Local (m)} & \textbf{Global (m)} \\
%             \midrule
%             \multirow{3}{*}{\centering Dataset0} & Baseline & -- & -- \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}-- & \cellcolor{lightgray}-- \\
%             & 78 GHz \toa & -- & -- \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset1} & Baseline & 1.370 & 2.458 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.059 & \cellcolor{lightgray}0.380 \\
%             & 78 GHz \toa & 0.058 & 0.121 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset2} & Baseline & 1.284 & 2.323 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.089 & \cellcolor{lightgray}0.186 \\
%             & 78 GHz \toa & 0.075 & 0.152 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset3} & Baseline & 1.363 & 2.404 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.058 & \cellcolor{lightgray}0.162 \\
%             & 78 GHz \toa & 0.058 & 0.127 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset4} & Baseline & 1.041 & 2.276 \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.179 & \cellcolor{lightgray}0.320 \\
%             & 78 GHz \toa & 0.061 & 0.131 \\
%             \bottomrule
%         \end{tabular}
%         }
%     \end{subtable}
%     \hfill
%     \begin{subtable}{0.45\textwidth}
%         \centering
%         \caption{MONO Inertial}
%         \resizebox{\linewidth}{!}{%
%         \begin{tabular}{c l cc}
%             \toprule
%             \textbf{Dataset} & \textbf{Configuration} & \textbf{Local (m)} & \textbf{Global (m)} \\
%             \midrule
%             \multirow{3}{*}{\centering Dataset0} & Baseline & -- & -- \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.096 & \cellcolor{lightgray}0.434 \\
%             & 78 GHz \toa & 0.076 & 0.306 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset1} & Baseline & -- & -- \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.112 & \cellcolor{lightgray}0.190 \\
%             & 78 GHz \toa & 0.121 & 0.370 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset2} & Baseline & -- & -- \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.217 & \cellcolor{lightgray}0.336 \\
%             & 78 GHz \toa & 0.197 & 0.649 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset3} & Baseline & -- & -- \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.063 & \cellcolor{lightgray}0.128 \\
%             & 78 GHz \toa & 0.063 & 0.123 \\
%             \cmidrule(lr){2-4}
%             \multirow{3}{*}{\centering Dataset4} & Baseline & -- & -- \\
%             & \cellcolor{lightgray}28 GHz \toa & \cellcolor{lightgray}0.102 & \cellcolor{lightgray}0.314 \\
%             & 78 GHz \toa & 0.102 & 0.150 \\
%             \bottomrule
%         \end{tabular}
%         }
%     \end{subtable}

% \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[htbp]
    \centering
   \caption[Comparison of SLAM Performance with \toa Integration]{Average Errors and Improvements for Different SLAM Modes. \\\textit{\footnotesize Note: For the monocular mode with \toa integration, results for Datasets 2 and 4  are calculated up to 75\,s and 65\,s respectively, as the system lost tracking beyond these durations.}}
    \label{tab:combined}

    % First Row of Subtables
    \begin{subtable}{0.49\textwidth}
        \centering
        \caption{RGB-D}
       \resizebox{1\linewidth}{!}{%
    \begin{tabular}{c l c c c}
        \toprule
        \textbf{Dataset} & \textbf{Configuration}
          & \textbf{Local (m)} & \textbf{Global (m)} & \textbf{Local Imp. } \\
        \midrule

        %------------------- Dataset0 -------------------
        \multirow{3}{*}{Dataset0}
            & Baseline
                & 0.064 & N/A{$^\ddagger$}    & -- \\
            & \cellcolor{lightgray}28 GHz \toa
                & \cellcolor{lightgray}0.066
                & \cellcolor{lightgray}0.237
                & \cellcolor{lightgray}\coloredpercent{-3.1} \\
            & 78 GHz \toa
                & 0.055 & 0.101 & \coloredpercent{14.1} \\
        \cmidrule(lr){1-5}

        %------------------- Dataset1 -------------------
        \multirow{3}{*}{Dataset1}
            & Baseline
                & 0.116 & N/A    & -- \\
            & \cellcolor{lightgray}28 GHz \toa
                & \cellcolor{lightgray}0.117
                & \cellcolor{lightgray}0.165
                & \cellcolor{lightgray}\coloredpercent{-0.9} \\
            & 78 GHz \toa
                & 0.117 & 0.133 & \coloredpercent{-0.9} \\
        \cmidrule(lr){1-5}

        %------------------- Dataset2 -------------------
        \multirow{3}{*}{Dataset2}
            & Baseline
                & 0.155 & N/A    & -- \\
            & \cellcolor{lightgray}28 GHz \toa
                & \cellcolor{lightgray}0.160
                & \cellcolor{lightgray}0.197
                & \cellcolor{lightgray}\coloredpercent{-3.2} \\
            & 78 GHz \toa
                & 0.148 & 0.158 & \coloredpercent{4.5} \\
        \cmidrule(lr){1-5}

        %------------------- Dataset3 -------------------
        \multirow{3}{*}{Dataset3}
            & Baseline
                & 0.095 & N/A    & -- \\
            & \cellcolor{lightgray}28 GHz \toa
                & \cellcolor{lightgray}0.102
                & \cellcolor{lightgray}0.149
                & \cellcolor{lightgray}\coloredpercent{-7.4} \\
            & 78 GHz \toa
                & 0.094 & 0.104 & \coloredpercent{1.1} \\
        \cmidrule(lr){1-5}

        %------------------- Dataset4 -------------------
        \multirow{3}{*}{Dataset4}
            & Baseline
                & 0.146 & N/A    & -- \\
            & \cellcolor{lightgray}28 GHz \toa
                & \cellcolor{lightgray}0.162
                & \cellcolor{lightgray}0.242
                & \cellcolor{lightgray}\coloredpercent{-11.0} \\
            & 78 GHz \toa
                & 0.164 & 0.171 & \coloredpercent{-12.3} \\
        % \cmidrule(lr){1-5}
        \bottomrule

        %----------------- Mode Average -----------------
        \multirow{3}{*}{\textbf{Mode Average}}
            & Baseline
                & \textbf{0.115} & N/A & -- \\
            & \cellcolor{lightgray}28 GHz \toa
                & \cellcolor{lightgray}\textbf{0.121}
                & \cellcolor{lightgray}\textbf{0.198}
                & \cellcolor{lightgray}\textbf{\coloredpercent{-5.2}} \\
            & 78 GHz \toa
                & \textbf{0.116} & \textbf{0.133} & \textbf{\coloredpercent{1.3}} \\

        \bottomrule
    \end{tabular}
        }
    \end{subtable}
    \hfill
      % First Row of Subtables
    \begin{subtable}{0.49\textwidth}
        \centering
        \caption{RGB-D Inertial}
       \resizebox{1\linewidth}{!}{%
    \begin{tabular}{c l c c c}
        \toprule
        \textbf{Dataset} & \textbf{Configuration}
          & \textbf{Local (m)} & \textbf{Global (m)} & \textbf{Local Imp. } \\
        \midrule
    \multirow{3}{*}{Dataset0} 
    & Baseline
        & 0.089 & N/A    & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.092
        & \cellcolor{lightgray}0.471
        & \cellcolor{lightgray}\coloredpercent{-3.4} \\
    & 78 GHz \toa
        & 0.075 & 0.276 & \coloredpercent{15.7} \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset1} 
    & Baseline
        & 0.119 & N/A    & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.118
        & \cellcolor{lightgray}0.206
        & \cellcolor{lightgray}\coloredpercent{0.8} \\
    & 78 GHz \toa
        & 0.118 & 0.315 & \coloredpercent{0.8} \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset2} 
    & Baseline
        & 0.216 & N/A    & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.231$^\dagger$
        & \cellcolor{lightgray}0.267
        & \cellcolor{lightgray}\coloredpercent{-6.9} $^\dagger$ \\
    & 78 GHz \toa
        & 0.366$^\dagger$ & 0.426 & \coloredpercent{-69.4} $^\dagger$ \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset3} 
    & Baseline
        & 0.065 & N/A    & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.064
        & \cellcolor{lightgray}0.134
        & \cellcolor{lightgray}\coloredpercent{1.5} \\
    & 78 GHz \toa
        & 0.062 & 0.125 & \coloredpercent{4.6} \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset4} 
    & Baseline
        & 0.108 & N/A    & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.105
        & \cellcolor{lightgray}0.321
        & \cellcolor{lightgray}\coloredpercent{2.8} \\
    & 78 GHz \toa
        & 0.105 & 0.168 & \coloredpercent{2.8} \\
% \cmidrule(lr){1-5}
\bottomrule

\multirow{3}{*}{\textbf{Mode Average}} 
    & Baseline
        & \textbf{0.095} & N/A & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}\textbf{0.94}
        & \cellcolor{lightgray}\textbf{0.280}
        & \cellcolor{lightgray}\textbf{\coloredpercent{0.42}} \\
    & 78 GHz \toa
        & \textbf{0.90} & \textbf{0.262} & \textbf{\coloredpercent{5.97}} \\
        \bottomrule

        % --------------------------- MONO SLAM Mode ---------------------------
        \end{tabular}
        }
    \end{subtable}

    \vspace{0.5cm}

    % Second Row of Subtables
    \begin{subtable}{0.49\textwidth}
        \centering
        \caption{MONO}
       \resizebox{1\linewidth}{!}{%
    \begin{tabular}{c l c c c}
        \toprule
        \textbf{Dataset} & \textbf{Configuration}
          & \textbf{Local (m)} & \textbf{Global (m)} & \textbf{Local Imp. } \\
        \midrule

\multirow{3}{*}{Dataset0} 
    & Baseline 
        & Failed    & N/A & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}Failed 
        & \cellcolor{lightgray}Failed 
        & \cellcolor{lightgray}-- \\
    & 78 GHz \toa
        & Failed    & Failed & -- \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset1} 
    & Baseline
        & 1.370 & N/A    & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.059
        & \cellcolor{lightgray}0.380
        & \cellcolor{lightgray}\coloredpercent{95.7} \\
    & 78 GHz \toa
        & 0.058 & 0.121 & \coloredpercent{95.8} \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset2} 
    & Baseline
        & 1.284 & N/A    & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.089
        & \cellcolor{lightgray}0.186
        & \cellcolor{lightgray}\coloredpercent{93.1} \\
    & 78 GHz \toa
        & 0.075 & 0.152 & \coloredpercent{94.2} \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset3} 
    & Baseline
        & 1.363 & N/A    & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.058
        & \cellcolor{lightgray}0.162
        & \cellcolor{lightgray}\coloredpercent{95.7} \\
    & 78 GHz \toa
        & 0.058 & 0.127 & \coloredpercent{95.7} \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset4} 
    & Baseline
        & 1.041 & N/A    & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.179
        & \cellcolor{lightgray}0.320
        & \cellcolor{lightgray}\coloredpercent{82.8} \\
    & 78 GHz \toa
        & 0.061 & 0.131 & \coloredpercent{94.1} \\
% \cmidrule(lr){1-5}
\bottomrule

\multirow{3}{*}{\textbf{Mode Average}} 
    & Baseline
        & \textbf{1.265} & N/A & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}\textbf{0.096}
        & \cellcolor{lightgray}\textbf{0.262}
        & \cellcolor{lightgray}\textbf{\coloredpercent{92.4}} \\
    & 78 GHz \toa
        & \textbf{0.063} & \textbf{0.133} & \textbf{\coloredpercent{95.0}} \\



            \bottomrule
        \end{tabular}
        }
    \end{subtable}
    \hfill
      \begin{subtable}{0.49\textwidth}
        \centering
        \caption{MONO Inertial}
       \resizebox{1\linewidth}{!}{%
    \begin{tabular}{c l c c c}
        \toprule
        \textbf{Dataset} & \textbf{Configuration}
          & \textbf{Local (m)} & \textbf{Global (m)} & \textbf{Local Imp. } \\
        \midrule

       \multirow{3}{*}{Dataset0} 
    & Baseline 
        & Failed & N/A & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.096
        & \cellcolor{lightgray}0.434
        & \cellcolor{lightgray}  \nagreenn \\
    & 78 GHz \toa
        & 0.076 & 0.306 &  \nagreen \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset1} 
    & Baseline 
        & Failed & N/A & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.112
        & \cellcolor{lightgray}0.190
        & \cellcolor{lightgray}  \nagreen \\
    & 78 GHz \toa
        & 0.121 & 0.370 &  \nagreen \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset2} 
    & Baseline 
        & Failed & N/A & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.217
        & \cellcolor{lightgray}0.336
        & \cellcolor{lightgray} \nagreen \\
    & 78 GHz \toa
        & 0.197 & 0.649 &  \nagreen \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset3} 
    & Baseline 
        & Failed & N/A & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.063
        & \cellcolor{lightgray}0.128
        & \cellcolor{lightgray} \nagreen \\
    & 78 GHz \toa
        & 0.063 & 0.123 &  \nagreen \\
\cmidrule(lr){1-5}

\multirow{3}{*}{Dataset4} 
    & Baseline 
        & Failed & N/A & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}0.102
        & \cellcolor{lightgray}0.314
        & \cellcolor{lightgray} \nagreen \\
    & 78 GHz \toa
        & 0.102 & 0.150 &  \nagreen \\
% \cmidrule(lr){1-5}
\bottomrule

\multirow{3}{*}{\textbf{Mode Average}} 
    & Baseline
        & \textbf{Failed} & N/A & -- \\
    & \cellcolor{lightgray}28 GHz \toa
        & \cellcolor{lightgray}\textbf{0.118}
        & \cellcolor{lightgray}\textbf{0.280}
        & \cellcolor{lightgray}\textbf{ \nagreen} \\
    & 78 GHz \toa
        & \textbf{0.112} & \textbf{0.320} & \textbf{ \nagreen} \\


            \bottomrule
        \end{tabular}
        }
    \end{subtable}

        \vspace{0.3em}
\begin{minipage}{\linewidth}
        {\fontsize{6}{9} \selectfont
            $\dagger$ Dataset2's RGB-D Inertial with \toa results were excluded from average calculations due to anomalous degradation. \\[-0.5em]
            $*$ The symbol INF indicates cases where \toa enabled successful tracking when the baseline failed.\\[-0.5em]
            $\ddagger$ N/A denotes baseline systems without global positioning capability.}
    \end{minipage}
\end{table}
